Resource Allocation in Laser-based Optical Wireless Cellular Networks

Optical wireless communication provides data transmission at high speeds which can satisfy the increasing demands for connecting a massive number of devices to the Internet. In this paper, vertical-cavity surface-emitting(VCSEL) lasers are used as transmitters due to their high modulation speed and energy efficiency. However, a high number of VCSEL lasers is required to ensure coverage where each laser source illuminates a confined area. Therefore, multiple users are classified into different sets according to their connectivity. Given this point, a transmission scheme that uses blind interference alignment (BIA) is implemented to manage the interference in the laser-based network. In addition, an optimization problem is formulated to maximize the utility sum rate taking into consideration the classification of the users. To solve this problem, a decentralized algorithm is proposed where the main problem is divided into sub-problems, each can be solved independently avoiding complexity. The results demonstrate the optimality of the decentralized algorithm where a sub-optimal solution is provided. Finally, it is shown that BIA can provide high performance in laser-based networks compared with zero forcing (ZF) transmit precoding scheme.

==> main.tex <==

\input{./1570730039.tex} %Preamble
\begin{document}
\frontmatter
\input{./IEEEtran.cls}
\input{./plot/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}


==> source files (2)/main.tex <==

\input{./1570730039.tex} %Preamble
\begin{document}
\frontmatter
\input{./IEEEtran.cls}
\input{./plot/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}

